Time-Optimal Online Replanning for Agile Quadrotor Flight

In this paper, we tackle the problem of flying a quadrotor using time-optimal control policies that can be replanned online when the environment changes or when encountering unknown disturbances. This problem is challenging as the time-optimal trajectories that consider the full quadrotor dynamics are computationally expensive to generate (order of minutes or even hours). We introduce a sampling-based method for efficient generation of time-optimal paths of a point-mass model. These paths are then tracked using a Model Predictive Contouring Control approach that considers the full quadrotor dynamics and the single rotor thrust limits. Our combined approach is able to run in real-time, being the first time-optimal method that is able to adapt to changes on-the-fly. We showcase our approach's adaption capabilities by flying a quadrotor at more than 60 km/h in a racing track where gates are moving. Additionally, we show that our online replanning approach can cope with strong disturbances caused by winds of up to 68 km/h.

==> Tables/baselines.tex <==
{
\renewcommand{\arraystretch}{1.5}
\begin{table*}[!htp]
    \centering
    \setlength{\tabcolsep}{3pt}
    \caption{A baseline comparison of different methods for drone racing}
    \label{tab:results_overview}
    \begin{tabular}{c c cc cc cc}
        \toprule
        \multirow{2}{*}{\begin{minipage}{5mm} Race\\Track\end{minipage}} & \multirow{2}{*}{\begin{minipage}{15mm}Simulation\\Environment\end{minipage}} 
        &  \multicolumn{2}{c}{MPCC~\cite{romero2021model}} 
        &  \multicolumn{2}{c}{RL~\cite{song2021autonomous}}
        &  \multicolumn{2}{c}{MPC~\cite{foehn2021CPC}}  \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
        & & Lap Time & Passing Dist. & Lap Time & Passing Dist. & Lap Time  & Passing Dist.  \\
        \hline
        \multirow{2}{*}{SplitS} 
        & Simple & 5.150 & 0.232  $\pm$ 0.174 & 5.074 & 0.172 $\pm$ 0.052  & x&x \\
        & BEM  & 5.234 & 0.361 $\pm$ 0.134 & 5.004 & 0.478  $\pm$ 0.101 & x&x \\
        \hline
        \multirow{2}{*}{Straight} 
        & Simple  & x&x & 0.557 & 0.115 $\pm$ 0.038  & x&x \\
        & BEM  & x&x & 0.589 & 0.080 $\pm$0.051 & x&x \\
        \hline
        \multirow{2}{*}{Vertical} 
        & Simple  & x&x & 0.793& 0.159 $\pm$ 0.053 & x&x \\
        & BEM  & x&x & 0.829 & 0.151  $\pm$ 0.048 & x&x \\
        \hline
        \multirow{2}{*}{AlphaPilot} 
        & Simple  & x&x & 5.33 & 0.198 $\pm$ 0.124  & x&x\\
        & BEM  & x&x & x&x  & x&x \\
        \bottomrule
    \end{tabular}
\end{table*}
}



==> Tables/racing_baselines.tex <==
{
\renewcommand{\arraystretch}{1.5}
\begin{table}[!htp]
    \centering
    \setlength{\tabcolsep}{3pt}
    \caption{Baselines}
    \label{tab:results_overview}
    \begin{tabular}{c|c|c|c}
        \toprule
        \rowcolor{Gray}
        Method & Environment & Lap Time ($\si{s}$) & Gate Passing Errors (\si{m})  \\
        \hline
        \multirow{2}{*}{MPCC} 
        & Simple & 5.150 $\pm$ 0.014 & 0.232 $\pm$ 0.174     \\
        & BEM & 5.234 $\pm$ 0.022 & 0.361 $\pm$ 0.134    \\
        \hline
        \multirow{2}{*}{MPC} 
        & Simple & 6.120 $\pm$  0.000 & $\pm$     \\
        & BEM & 6.120 $\pm$ 0.000 & $\pm$    \\
        \hline
        \multirow{2}{*}{RL (Ours)} 
        & Simple & 5.184  $\pm$ 0.030  &  0.121 $\pm$ 0.058    \\
        & BEM & 5.216 $\pm$ 0.011  & 0.367 $\pm$ 0.201    \\
        % \hline
        % \multirow{2}{*}{TCN (Ours)} 
        % & Simple & 5.235 $\pm$ 0.009 &  0.094 $\pm$ 0.030     \\
        % & BEM & 5.242 $\pm$ 0.021 & 0.498 $\pm$ 0.233    \\
        % \hline
        % \multirow{2}{*}{RNN (Ours)} 
        % & Simple & 5.180 $\pm$ 0.014 & 0.111 $\pm$ 0.042    \\
        % & BEM & 5.250 $\pm$  0.015 & 0.451 $\pm$ 0.217    \\
        \bottomrule
    \end{tabular}
\end{table}
}


